Dias: Dynamic Rewriting of Pandas Code

In recent years, dataframe libraries, such as pandas have exploded in popularity. Due to their flexibility, they are increasingly used in ad-hoc exploratory data analysis (EDA) workloads. These workloads are diverse, including custom functions which can span libraries or be written in pure Python. The majority of systems available to accelerate EDA workloads focus on bulk-parallel workloads, which contain vastly different computational patterns, typically within a single library. As a result, they can introduce excessive overheads for ad-hoc EDA workloads due to their expensive optimization techniques. Instead, we identify program rewriting as a lightweight technique which can offer substantial speedups while also avoiding slowdowns. We implemented our techniques in Dias, which rewrites notebook cells to be more efficient for ad-hoc EDA workloads. We develop techniques for efficient rewrites in Dias, including dynamic checking of preconditions under which rewrites are correct and just-in-time rewrites for notebook environments. We show that Dias can rewrite individual cells to be 57$\times$ faster compared to pandas and 1909$\times$ faster compared to optimized systems such as modin. Furthermore, Dias can accelerate whole notebooks by up to 3.6$\times$ compared to pandas and 26.4$\times$ compared to modin.

==> APP_exper_setup.tex <==
\section{Details on the Experimental Setup}

\paragraph{\textbf{Machine}}

\begin{itemize}
    \item \textbf{CPU}: AMD Ryzen 9 5900X 12-Core, clocked at 3.7 GHz
    \item \textbf{RAM}: 32 GB DRAM
    \item \textbf{SSD}: Samsung 980 PRO
    \item \textbf{OS}: Ubuntu 22.04.1 LTS
    \item \textbf{Quiescing Settings}:
        \begin{itemize}
            \item Boot in terminal mode
            \item Disable turbo boost
            \item Disable frequency scaling
        \end{itemize}
\end{itemize}

We picked this as a conventional consumer machine, except for the SSD which is unconventionally fast.

\paragraph{\textbf{Python/Pandas Setup}}
\begin{itemize}
    \item Python: 3.10.6
    \item IPython: 8.5.0
    \item Numpy: 1.23.4
    \item Pandas: 1.5.1
\end{itemize}

\paragraph{\textbf{Benchmark}}

We disabled some code in these notebooks that we consider out of scope. In particular:
\begin{itemize}
    \item Networking or Shell code, i.e., cells like \code{pip install} or like \code{nltk.download()}.
        \begin{itemize}
            \item This means that to reproduce our experiments, you may need to run the original notebook once e.g., to download the required \code{nltk} dataset.
        \end{itemize}
    \item Plotting and machine-learning code
    \item IPython magic functions because our tool can only handle valid Python code. For these notebooks, we only had to remove \code{\%matplotlib inline}.
\end{itemize}


==> figures/alg_remove_axis_1.tex <==
% Thanks to Hydride team. Got part of the latex from there.

% It's not an algorithm but I liked the \begin{algorithm} format.
\floatname{algorithm}{Algorithm}

%%\renewcommand{\algorithmiccomment}[1]{\hfill\eqparbox{COMMENT}{#1}}
\renewcommand{\algorithmiccomment}[1]{\bgroup\hfill\footnotesize//~#1\egroup}
\algrenewcommand\algorithmicindent{1.0em}%

\begin{algorithm}[t!]
\caption{Preconditions for RemoveAxis1}
\label{alg:remove-axis-1-preconds}
\small{
\begin{algorithmic}[1]

\Function{IsCompatibleSub}{astNode}
  \State \textit{// Return True if astNode is a Subscript with}
  \State \textit{// Name for .value and Constant(str) for .slice.}
\EndFunction

\Function{CanRemoveAxis1}{funcBody, arg0Name}
\State theOneSeries : string = \textbf{None}

\State allowedNodes = \{ \\
  Return, For, While, If, Pass, Break, Continue  \\
  BoolOp, BinOp, UnaryOp, IfExp, Dict, Set, Compare, Constant, \\
  Subscript, Name, List, Tuple, Slice, Load
\}

\ForAll{[n \textbf{in} AstWalk(funcBody) \textbf{if} n \textbf{is} ast.Name]}
  \State parent := n's parent in the AST
  \If{type(n) not in allowedNodes \textbf{or} \\
      \hspace{25.2pt} name.id != arg0Name \textbf{or} \\
      \hspace{28pt}\textbf{not} IsCompatibleSub(parent)}
    \State \Return \textbf{False}
  \EndIf
  \State theSeries := parent.slice.value
  \If{theOneSeries \textbf{is not None and} \\
      \hspace{25.2pt} theOneSeries != theSeries}
    \State \Return \textbf{False}
  \EndIf
  \State theOneSeries := theSeries
\EndFor
\State \Return theOneSeries \textbf{is not None}

\EndFunction
\end{algorithmic}
}
\end{algorithm}

\setlength{\textfloatsep}{15pt}


==> figures/columnar.tex <==
\begin{figure}
  \begin{subfigure}[b]{0.45\columnwidth}
    \begin{minipage}{\linewidth}%
\begin{minted}[bgcolor=light-gray]{python}
def foo(row):
  if row['Fare'] > 10:
    return True
  return False

df.apply(foo, axis=1)
\end{minted}
\end{minipage}
    \caption{Row-Mjaor}
    \label{fig:row-major}
  \end{subfigure}
  \hfill %%
  \begin{subfigure}[b]{0.45\columnwidth}
    \begin{minipage}{\linewidth}%
\begin{minted}[bgcolor=light-gray]{python}
def foo(fare):
  if fare > 10:
    return True
  return False

df['Fare'].apply(foo)
\end{minted}
\end{minipage}
    \caption{Columnar}
    \label{fig:columnar}
  \end{subfigure}
  \caption{Row-Major vs Columnar Access}
\end{figure}

==> figures/extended/no_sliced_exec.tex <==
\begin{figure}[!h]
  \centering
  \includegraphics[width=\columnwidth]{figures/extended/sources/no_sliced_exec.pdf}
  \caption{Corresponding to Figure~\ref{fig:no_sliced_exec}. We see that sliced
  execution is still worth the engineering burden.}
  \label{fig:ext:no_sliced_exec}
\end{figure}


==> figures/lst_patt_match.tex <==
% Thanks to Hydride team. Got part of the latex from there.

% It's not an algorithm but I liked the \begin{algorithm} format.
\floatname{algorithm}{Listing}

%%\renewcommand{\algorithmiccomment}[1]{\hfill\eqparbox{COMMENT}{#1}}
\renewcommand{\algorithmiccomment}[1]{\bgroup\hfill\footnotesize//~#1\egroup}
\algrenewcommand\algorithmicindent{1.0em}%

\begin{algorithm}[t!]
\caption{A Sketch of \system{}' Pattern Matcher}
\label{lst:patt-match}
%%\akash{Algorithm modified. Font size is smaller now and comments are in the same line as the pseudocode}
\normalsize{
\begin{algorithmic}[1]
\Function{LambdaSubstrSearch}{stmt}

\State \textit{// Return True if stmt is a ast.Lambda}
\State \textit{// that performs substring search.}

\EndFunction
\Function{PatternMatch}{stmt}
\ForAll{node \textbf{in} stmt} 
    \If{node \textbf{is} ast.Call}
        \If{node.func.attr = "apply"}
            \State arg0 $\gets$ node.func.args[0]
            \If{\Call{LambdaSubstrSearch}{arg0}}
                \State \Return SubstringSearchApply
            \EndIf
            \If{isinstance(arg0, ast.Name)}
              \If{node.func.args[1] \textbf{is} axis=1}
                \State \Return ApplyAxis1
              \EndIf
            \EndIf
        \EndIf
    \EndIf
\EndFor
\State \Return \textbf{None}
\EndFunction

\end{algorithmic}
}
\end{algorithm}
\setlength{\textfloatsep}{15pt}


==> figures/multi_stmt_patt.tex <==
\begin{figure}
  \begin{subfigure}[t]{\columnwidth}
\begin{minted}[bgcolor=light-gray]{python}
df['original_price'] = 
  df['original_price'].str.split('$')
df['original_price'] = df['original_price'].str[1]
\end{minted}
  \caption{Original}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{\columnwidth}
\begin{minted}[bgcolor=light-gray]{python}
res = []
col = df['original_price']
for s in col.tolist():
    spl = s.split('$')
    res.append(spl[1])
df['original_price'] = pd.Series(res, ser.index)
\end{minted}
  \caption{Rewritten}
  \end{subfigure}
  \caption{An example of a multi-statement pattern (omitting runtime preconditions)}
  \label{fig:multi_stmt_patt}
\end{figure}

==> figures/no_sliced_exec.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\columnwidth]{figures/sources/no_sliced_exec.pdf}
  \caption{Slowdowns on whole notebooks without sliced execution. Disabling sliced execution leads to slowdowns and no significant speedups. }
  \label{fig:no_sliced_exec}
\end{figure}

==> figures/ocaml_local_binding.tex <==


\begin{figure}
  \begin{minted}[bgcolor=light-gray,escapeinside=||]{ocaml}
test(mod_x(), 
  let tmp = foo().read_x() in
    if type(tmp) == pd.|Series| 
      then tmp.nsmallest()
      else tmp.sort_values().head())
  \end{minted}
    \caption{A local binding in the style of OCaml.}
    \label{fig:ocaml-local-binding}
\end{figure}

==> figures/precond_naive.tex <==
\begin{figure}
\begin{minted}[bgcolor=light-gray,escapeinside=||]{python}
tmp = @{called_on}
if type(tmp) == pandas.Series:
  tmp.nsmallest()
else:
  tmp.sort_values().head()
\end{minted}
  \caption{A naive precondition check.}
  \label{fig:sort-values-precond-naive}
\end{figure}

==> figures/precond_naive2.tex <==
\begin{figure}
\begin{minted}[bgcolor=light-gray,escapeinside=||]{python}
tmp = foo().read_x()
if type(tmp) == pandas.Series:
  test(mod_x(), tmp.nsmallest())
else:
  test(mod_x(), tmp.sort_values().head())
\end{minted}
  \caption{An incorrect precondition check when having a nested expression.}
  \label{fig:sort-values-precond-naive2}
\end{figure}

==> figures/sort_values_formal.tex <==
\begin{figure}

\begin{mathpar}
\inferrule
{(\code{@\{name\}}, \Gamma_{1}) \Downarrow Obj, \Gamma_{2} \\ (\code{type(Obj)}, \Gamma_{2}) \Downarrow \code{DataFrame}, \Gamma_{2} \\ (LHS, \Gamma_{1}) \Downarrow VLHS, \Gamma_{4} \\ (RHS, \Gamma_{1}) \Downarrow VRHS, \Gamma_{5} }
{VLHS = VRHS \wedge \Gamma_{4} = \Gamma_{5}}
\end{mathpar}

    \caption{Formal Semantics the Rewrite Rule in Figure \ref{fig:sort-values-rule}}
    \label{fig:sort-values-formal}
\end{figure}

==> limitations.tex <==

\section{Limitations}

\paragraph{\textbf{Generalizability of Patterns}} Suppose that we need $P$
patterns to rewrite cells in $N$ random notebooks and consider the ratio of $P$
over $N$. We say that the patterns generalize well if as $N$ gets larger, then
this ratio gets smaller, meaning, $N$ grows much faster than $P$. The current
patterns do not generalize well. We rewrite 10 notebooks but we needed to code
10 patterns to achieve this. If we pick 10 \emph{other} random notebooks, the
results may not be the same. Of course, $N = 10$ is very small to make an
inductive argument that this is the rule as $N$ increases. Nonetheless, we
currently have no evidence that the patterns will eventually generalize.

\paragraph{\textbf{Engineering Effort}} Currently, there is a non-trivial effort
required to both find and code the patterns and \system{} does not provide any
automation for either. We hope in the future to improve it on both aspects. The
latter is more tractable and it would probably require a framework in which one
can succinctly express patterns. The former is much harder. Finding patterns
requires both reasoning about program semantics (an infamous hurdle in Python)
and cost-modeling equivalent versions.

% \stef{Well, I was gonna add interoperability with Pandas replacements as a
% limitation but in fact, one can disable patterns and leave only those that go
% from Pandas to Pandas}

\paragraph{\textbf{Effective Use of Hardware}}

The speedups \system{} provides do not scale in a way aligned with modern
hardware trends i.e., hardware replication (e.g., multi-core machines or
distributed storage). Adding more cores, machines or disks will have no effect,
as it does for Python and \code{pandas}. Nevertheless, even though in this paper we
explored the surprising direction of going from \code{pandas} to Python, the inverse,
i.e., going from Python to \code{pandas}, still has performance benefits. This is
something we hope to explore in the future. %using rewriting.

